Bid Shading by Win-Rate Estimation and Surplus Maximization

This paper describes a new win-rate based bid shading algorithm (WR) that does not rely on the minimum-bid-to-win feedback from a Sell-Side Platform (SSP). The method uses a modified logistic regression to predict the profit from each possible shaded bid price. The function form allows fast maximization at run-time, a key requirement for Real-Time Bidding (RTB) systems. We report production results from this method along with several other algorithms. We found that bid shading, in general, can deliver significant value to advertisers, reducing price per impression to about 55% of the unshaded cost. Further, the particular approach described in this paper captures 7% more profit for advertisers, than do benchmark methods of just bidding the most probable winning price. We also report 4.3% higher surplus than an industry Sell-Side Platform shading service. Furthermore, we observed 3% - 7% lower eCPM, eCPC and eCPA when the algorithm was integrated with budget controllers. We attribute the gains above as being mainly due to the explicit maximization of the surplus function, and note that other algorithms can take advantage of this same approach.

==> Improvements.tex <==
\textcolor{red}{[Tian's bucketing strategy]}


\cBl


\subsection{Algorithm Comparisons}
\begin{itemize}
    \item \textit{biderr + penalty} Already running..
    \item \textit{SSP WinRate Maintainer} Either implement algorithm based on the Logistic that finds that point at which winrate>=0.9 (target), OR just use AdX as the comparison.
    \item \textit{AdX Anonymized SSP} We'd call this an Anonymous SSP bid shader. Show the performance of this algorithm. Ideally our algorithm would perform better than it. 
    \item \textit{Other} Other algorithms running in production we can show
    \end{itemize}  
\cG

\cBl
\subsection{Over-sampling Issue / Surplus Error / Weighted Training (Unique to domain)}
\begin{itemize}
\item \textit{Observation weights} One of the characteristics of this problem, is fitting the logistic based on all points tends to result in a "crowding" / over-weight of observations in the low (losing) region of the curve. Simply stated, there is an incentive to bid low in case the advertiser wins the impression for a low price. But this means more losing observations than winning (usually). There are fewer bids that are high priced. This means that the fit "overweights" / heavily weights the observations that are low on the curve, ensuring that those points are fit with low error. However would be more important in practice to have low error in the region of the curve where the bidder is more likely to submit their bid. One method is to calculate Pr(bidsubmitted | bidder=b and pattern=x), and then weight error by this metric. This will tend to force the regions of the curve that have historically been more likely to be bid to have a better fit.
\end{itemize}
\paragraph{}
\begin{itemize}
Weighting was recently added to Pyspark's Logistic regression. Below is the parameter to add:
\begin{verbatim}
new LogisticRegression().setWeightCol("classWeightCol")
.setLabelCol("label")
.setFeaturesCol("features")
https://issues.apache.org/jira/browse/SPARK-9610
https://github.com/apache/spark/pull/7884
\end{verbatim}
\end{itemize}


\subsection{Enhanced Logistic (unique to domain)}
\begin{itemize}
\item \textit{Enhanced Landscapes} While the logistic is a reasonable model for the win probability landscape, it is, however an approximation. Real win probability landscapes exhibit a range of characteristics that should be taken advantage of in practice if possible. One prominent feature of these curves is the tendency to see crowdings of winning bids around round numbers. This has been speculated as possibly due to the presence of human-set floor prices on the auction, as well as bidders that bid fixed CPMs. In order to take advantage of these features, we augment the logistic curve fitting proces, and add a short list of salient price features..
\end{itemize}

\subsection{Coordinated Bidding (Adjustment to avoid self-competition in First Price Auctions)}

\begin{itemize}
\item \textit{Coordinated bidding} Many large DSPs may represent multiple advertisers and have a fiduciary responsibility to minimize the cost to advertisers bidding on the auction. DSPs that have multiple customers can actually coordinate their bids to avoid escalating the price in first price auctions \cite{kitts2005cooperative}. Estimates for the percentage of bidders that are DSP controlled ranges from about 8\% to about 34\%. In order to implement collusive bidding, perform all the same computations, however, when calculating the minimum-bid-price-to-win (winning price), calculate this having de-duplicated DSP controlled bidders. Then everyone is pricing towards the "price needed to exceed /other/ bidders". Collusion won't work if some of the DSP bidders aren't controlled by this de-duplication process, or are in other buckets etc. 
\end{itemize}

\cB



\subsection{Reproduceability}
\begin{itemize}
\item \textit{Reproduceability}. May be able to connect this to a data release I've been working on, and show that this method performs well against others. This would be publicly available. 
\end{itemize}


\subsection{Domain Unique Issues and Performance}
\begin{itemize}
\item \textit{Domain unique issues}. Auction forecasting is challenging. Other DSPs have incentive to engage in strategic forecasting behavior also, creating instability in the auction.  
\item \textit{Suitability for domain}. Aspects of algorithm designed to deal with strategic issues. One conclusion about auction theory would be that the faster DSP and the one that is better able to predict the auction state, the better that DSP will perform. May need to have a "Fast modeling component" that is able to better judge the current state of the auction. ie. this component would be able to react to rapid changes from other DSPs. 
\end{itemize}



%\cBl
%\begin{figure}
%\centering
%\subfloat{\includegraphics[width=0.48\columnwidt%h]{images/shaded_factor_distributions_Logistic_v%rs_SSP.png}}\\
%
%\caption{Shading distributions for Logistic %approach (top), direct surplus maximization %(middle) and SSP winrate maintenance (bottom)}
%
%\label{fig:shading_distributions}
%\end{figure}

% \cB



\subsection{Low-price Inventories}
\textcolor{red}{[Not Needed]}
In practice surplus is not a direct metric that a DSP platform evaluates. The belief is that improvement in surplus will bring more values to the advertisers and eventually improve other metrics such as eCPM, eCPC and eCPA. However, we have observed that in practise that is not the case: by blindly applying a shading algorithm to all bid requests result in higher (worse) eCPM. The cause is that, shading on ad inventories with low bid price and/or inventory cost does not contribute much to the overall surplus, but it impacts eCPM greatly. In other words, an aggressive bid shading algorithm would shade too much on low-price inventories and thus lose opportunities of a significant amount of impressions. Thus for practice consideration care must be taken for low-price inventories.




\subsection{Offline experiments and analysis}
In this section, we will analyze the performance of the machine learning based approaches using both regression metrics and demand platform performance metrics in an offline setting using the retrospective analysis. This will allow us to very easily characterize algorithmic performance on the available data, as well as to do a deeper dive into goal type performance analysis and fine-tuning of hyperparameters.

\subsubsection{Machine learning based approaches and their performance}
On the described dataset we train the three mentioned machine learning based approaches, characterize their regression performance and finally compare their individual improvements against the production baseline.
The regression performance is aimed to evaluate how well the algorithms fit the data, which, in the setup proposed in this study, means predicting the competitive landscape, a very difficult task indeed given a large number of demand platforms and highly variable number of external lines and ads that could potentially target the current opportunity. This is clearly reflected in lower $r^2$ values on all algorithms, however its positivity shows that models can still capture some of the large variablity of the bid shading signal.


For the regression metrics (Figure~\ref{fig:exp_main_regression}) we can see that there is a clear distinction among the algorithms (especially in terms of the $r^2$ metric) where the MLP approach had the worst performance, while the proposed FM approach had the best performance. We suspect that the combination of existing features does not provide as much as predictive information as does modeling heterogeneity of each feature (i.e. through the feature learning layer in the FM model).
\begin{figure}[!ht]
	\centering
% 	\includegraphics[width=0.30\textwidth]{images/exp_main_regression.png}
% 	\caption{MSE and $r^2$ performance metrics for the three machine learning based approaches.}
	\label{fig:exp_main_regression}
\end{figure}

More interesting results are shown in Table~\ref{tbl:exp_main_performance}, where the three machine learning based approaches are directly compared against the non-linear bid shading used in production on surplus, spend, win rate and CPM metrics. Across the board we can see that each machine learning based approach outperforms the nonlinear bid shader on surplus, total spend and win rate. However, the CPM metric is always higher. The percentage increase in the CPM is of lesser importance than its absolute value (it is also directly controlled in several goal type lines such as eCPM) and the hyperparameters of the algorithms (in particular the $\gamma$ parameter) are tuned to yield lowest CPM increase for the surplus improvement (detailed analysis is provided in Section~\ref{sec:gamma_tuning}).
\begin{table}[!ht]
% \begin{tabular}{lcccc}
% \toprule
% & Surplus imp. & Spend imp. & CPM inc. & Win rate impr.       \\
% \midrule
% LR           & 17.20\%            & 128.63\%   & \textbf{67.56\%}   & \textbf{36.40\%} \\
% MLP          & 16.18\%            & 136.67\%   & 73.85\%   & 36.12\% \\
% FM           & \textbf{18.57\%}            & \textbf{133.02\%}   & \textit{70.82\%}   & \textbf{36.40\%} \\
% \bottomrule
% \end{tabular}%
% \caption{Improvements across surplus, total spend, win rate and increase of the CPM expressed in percentages over the nonlinear bid shading production baseline as obtained by the three machine learning based approaches.}
\label{tbl:exp_main_performance}
\end{table}
The highest surplus, spend and win rate improvements are obtained with the factorization machine approach yielding a bit higher CPM increase than of the linear regression which had the best CPM performance among the machine learning based approaches. MLP algorithm had the poorest performance across these metrics, however, it was still able to boost the performance of the nonlinear bid shading algorithm.


\subsubsection{Performance analysis per demand platforms' goal type}
Further characterization of the performance of different models can be done per goal types lines are optimizing towards, primarily because of the two following reasons: 1) the bid price calculation is slightly different for each goal type and 2) each goal type can have different control signals. 
The goal types of particular interest on the platform were \textit{None} goal type and five CP-X goals -- CPC(click), CPA(action), CPCV(completed view), CPViewI(viewed impressions) and eCPM(mile or 1000 impressions). The ratio of the goal types of interest in our test sample is provided in Figure~\ref{fig:goal_type_ratio}.
\begin{figure}[!ht]
	\centering
% 	\includegraphics[width=0.3\textwidth]{images/goal_type_ratio.png}
% 	\caption{Ratio of goal type opportunities of interest in the test set sample.}
	\label{fig:goal_type_ratio}
\end{figure}

As in the previous section, we separate the evaluation of algorithms into regression and platform performance metrics and show the performance of the proposed Factorization Machine model as the best performing model. Regression metrics per goal type are shown in Table~\ref{fig:exp_fm_goal_type_regression2}. We can see that regression performance does vary per line type, where the performance is most aligned with the overall results for two dominant goal types -- None and CPA. It is expected for the performance numbers to drop for goal types that have a very small yet non-negligible share of the serving opportunities due to the inherent noise of the problem.
\begin{figure}[!ht]
	\centering
% 	\includegraphics[width=0.43\textwidth]{images/exp_fm_goal_type_regression2.png}
% 	\caption{MSE and $r^2$ performance metrics for the Factorization Machine algorithm broken down by the goal type.}
% 	\label{fig:exp_fm_goal_type_regression2}
\end{figure}

Furthermore, once we analyze the performance of the FM-based bid shading approach against the nonlinear production baseline across surplus, total spend, win rate and CPM we can clearly see that there are improvements across the board with an acceptable increase of the average CPM.
\begin{figure}[!ht]
	\centering
% 	\includegraphics[width=0.5\textwidth]{images/exp_fm_goal_type_performance.png}
% 	\caption{Improvements across surplus, total spend, win rate and increase of the CPM expressed in percentages over Nonlinear bid shading production baselines obtained by the Factorization Machine model broken down by the goal type.}
	\label{fig:exp_fm_goal_type_performance2}
\end{figure}
Moreover, as the highest increase we observe is for the CPA goal which typically has the highest prices, we can concur that better shading can deliver gains in practice for advertisers targeting sophisticated, rare, and high-priced goals. But also for goal types with smaller values such as CPM, or even CPC, where shading has fewer degrees of freedom to pick and chose how to adjust the price we can clearly see that there is added value.


As a result of this analysis, we can concur that the FM model provides a clear advantage over the production model across different goal types and that the performance stability is simply subject to the goal type ration in a given sample.


\subsubsection{Effect of asymmetric loss function}
As we argued above that using asymmetric loss function can incentivize algorithm to optimize towards the higher surplus, we have conducted a simple experiment on linear regression model to inspect the impact of using a different loss function than standard mean squared error.

Figures~\ref{fig:assym_regression} and ~\ref{fig:assym_performance} show performance comparisons of the two loss functions for regression and performance metrics, respectively. As expected, we can observe that there is a slight degradation of regression metrics when using the asymmetric loss function. However, the purpose of using the asymmetric loss function is to improve the surplus metric which it successfully does, while also having a smaller CPM values (which causally yield smaller total spend and win rate). The fine tuning of the parameter in the asymmetric loss function was made to obtain the smaller CPM value increase, and the results with chosen parameter are compared against default mean squared error loss in this experiment.
\begin{figure}[htp]
	\centering
% 	\subfloat[Regression metrics]{\label{fig:assym_regression}\includegraphics[width=30mm]{images/exp_lr_assym_regression.png}}\hspace{3mm}% % or \hspace{0.3\textwidth}
% 	\subfloat[Performance metrics (percentages)]{\label{fig:assym_performance}\includegraphics[width=50mm]{images/exp_lr_assym_performance.png}}
% 	\caption{Linear Regression comparison for regular mean squared error and assymetric loss functions for standard regression metrics and demant platform performance metrics. Without loss of predictive performance simple linear model is capable of yielding higher total surplus at a smaller CPM increase controlled by the gamma value ($\gamma = 0.2$).}
	\label{fig:mse_assym}
\end{figure}

\subsubsection{Using parameter $\gamma$ to control the CPM}
\label{sec:gamma_tuning}
Finally we show the line search results of choosing the $\gamma$ parameter to control the CPM increase in performance analysis. We choose the best performing FM algorithm for this task, and searched for the best $\gamma$ parameter by increments of $0.2$. In the world of selected performance parameters, as discussed above they are often at odds with one another, i.e. to have a bigger total spend and win rate you might have to pay more per opportunity. The obvious optimal performance shift would be to increase surplus while decreasing the CPM, however empirically such outcomes are very rare, thus we try to control the levels various metrics to accommodate others. In our case, we strive to obtain the least possible CPM increase under the current setup. It should be noted that for some lines, there are controllers that control the CPM value (i.e. eCPM line) but for others there is no such dedicated controller thus it is very important to select good generic parameter values with respect to CPM increase.


For example, if the event is a so-called conversion (e.g. a online purchase) then $v_i = pCVR_i *event\_value$, where $pCVR_i$ is the estimated probability of a conversion event being associated to the impression, and $event\_value$ is the monetary value of such conversion event. Finally, the constraint is placed on the optimization function to ensure that the total sum of impression costs to the advertiser $c_i$ does not exceed the budget $B$ defined for the same time window.

The objective above should result with the desired $v_i$ as the value of the impression, and submitting it is the optimal strategy in GSPs according to Vickrey property \cite{wilkens:cinderella}. However due to additional considerations such as pacing and the fear of bid value miss-calibration or overpaying the final bid submitted $b_i$ is often calculated as:
\begin{equation}
	b_i = f(\alpha * v_i),
\end{equation}

where $\alpha$ is a multiplicative parameter that controls the delivery of a line, i.e. with respect to the delivery pacing \cite{Grislain2019}, and function $f$ represents optimal bidding strategy. It was shown that for second-price auctions (when the equilibrium bidding strategy is truthful) with the correct setting of $\alpha$, $f$ can be a simple linear function\footnote{\url{https://observablehq.com/d/9d739b2bc5b22bd8}, accessed January 2020}. Depending on the auction type, $b_i$ can be unshaded (annotated with $b_i^u$) or shaded.

We can observe that deciding on the maximum bid is a function of three main components optimized through eq.~\ref{eq:bidding}. 





\cG

\subsection{Supply-side bid shading algorithms}

The shift from second to first-price auctions was extremely rapid, and many advertisers may have difficulty calculating shading adjustments. To ease the transition to first-price, a range of ad exchanges have begun to offer "default bid shading services" to help advertisers who might struggle to implement their own algorithm. Examples include Google's ADX, which offers a special ``Bid Translation Service'' to map advertiser private value bids to the first-price suitable, shaded, bids ~\cite{google:rtb}; Rubicon's ``Estimated Market Rate'' for providing shading for advertiser bids ~\cite{rubicon:EMR}; and AppNexus's ``Bid Price Optimization'' system ~\cite{appnexus:BPO}. These services are designed to shade high, private-value-like bids down to a price at which the advertiser continues to win at an equivalent rate, but with a less egregious price. While this is a useful outcome for supply-side platforms, since it ensures impressions continue to sell, whilst avoiding what might be otherwise be considered "price gouging", it is most certainly not utility maximizing for advertisers. These services are only sometimes available, and Google has said publicly that it plans to discontinue its service once demand platforms' bid shading efforts have become sufficiently mature.

\subsection{Segmented, non-linear shading algorithm}
One approach that is simple but effective, is to estimate the optimal bid shading ratio using parametric functions of the unshaded bid. The function parameters are either tuned manually, or algorithmically, based on a feedback mechanism that tries to maximize surplus. Parameters are trained for each unique inventory segment, which is represented as a combination of salient inventory properties such as seller exchange, top level domain, and so on. For each of these inventory segments, historical surplus data is fed back to an algorithm that adjusts parameter values iteratively, attempting to maximize surplus for that segment. The parameter fitting can be done using gradient descent, recursive least squares, or other approaches.

As a benchmark for the new methodology proposed in this paper, the following parametric function used in production by the DSP system was considered for both offline and online experiments:
\begin{equation}
    b_i=f(b_i^u) = \begin{cases}
            \log \frac{1 + u_1 * u_2 * b_i^u}{u_2} & u_2 > 0\\ 
            b_1 * b_i^u & \text{otherwise}
        \end{cases}
\end{equation}
where $u_1, u_2, b_1$ are the parameters, and $b_i^u$ is the unshaded bid. The algorithm used to adjust the parameters was a recursive least square methodology and segments were defined as the combination of exchange, top level domain, device and layout.

One drawback of the above Segment-based, Nonlinear approach, is that segments have to be predetermined and finding a suitable segment definition requires substantial analysis without being able to provide optimality guarantees.  Another disadvantage is that information across segments is not shared, which is a problem for segments that do not have enough traffic. 



\cBl
%% Remove this section after we decide what we like for the title
Original title:
\paragraph{}
A Unified Approach to Bid Shading for First-Price Auctions \paragraph{}
Comment: didn't think "Unified" was an ideal description, as it sounds like the model introduced below does "everything". Really the approach below is more of a "model based" approach - it makes a strong assumption about win probability following a logistic distribution, and fits to that distribution. 
\paragraph{}
Alternative Possible Titles: 
\paragraph{}
A Model-Based Approach to Bid Shading for First Price Auctions
\paragraph{}
A Machine Learning Approach to Bid Shading for First Price Auctions
\paragraph{}
An Auction Forecasting Approach to Bid Shading for First Price Auctions
\paragraph{}
A Predictive Approach to Bid Shading for First Price Auctions
\paragraph{}
Bid Shading in First Price Auctions by Forecasting Clearing Prices
\paragraph{}
Bid Shading in First Price Auctions by Adversarial Price Forecasting
\paragraph{}Another comment: There's an adversarial aspect of this that I think the reviewers would like if we were to add it - if we introduced features that were related to the behavior of other DSPs on the auction. We can't really see the other DSPs, but we can see side-effects in terms of the clearing price by time-of-day and day-of-week...
Perhaps if the model was "looking for" adversarial behavior - which would be a fairly rapid change in clearing prices...
\cB







**** HOLD OUT SET PERFORMANCE: SHOW THAT INCLUDING THE ZEROS LEADS TO HIGHER PROFIT CAPTURE

**** TRIAL: IMPLEMENT A CONSTRAINED VERSION: TRY SETTING DERIVATIVES SUCH THAT IF EVALUATION AT BID=0 LEADS TO WIN>0 THEN HIGH ERROR

**** GENERAL COMMENT: IF WE HAVE MINBIDTOWIN THEN WHY BOTHER WITH THE FLOOR PRICE? SURELY WE COULD JUST CREATE AS MANY OBSERVATIONS AS WE WANTED

**** THROUGHOUT THERE ARE OFTEN CALCULATIONS OF POTENTIAL PROFIT ETC WHICH USE THE MINBIDTOWIN. HOW WOULD EVERYTHING CHANGE IF THIS DOESN’T EXIST




Simulations


TRIALS TO COMPLETE:

\% of optimal training (profitscalar / potential)
LOGISTIC PROFIT CAPTURED TEST SET
WEIGHTED DERIVATIVES BY SURPLUS
-	SURPLUS WEIGHTED
-	POTENTIAL SURPLUS WEIGHTED
CASE PROFIT MAXIMIZER
SELECTED BID AT MAX PROFIT MAXIMIZER
ADD WIN OVERSAMPLING
ADD ZERO INTERCEPT CASES

ALL OF THE ABOVE ON TEST SET AFTER MAXIMIZATION



Implementation



Insights

Variables and Variable values
Time of day variables



Metrics

Surplus
\% of optimal 
\% of optimal impressions, spend, surplus


Win-rate results

Training algorithm make use of \% of optimal?



\cB


%(2) \textbf{Feature Generation} Unique top level page domains, devices, and other characteristics of the bid requests are enumerated and converted into 0-1 variables for use in training.


How is the model being trained and uploaded?
\begin{itemize}
    \item \textit{Training pipeline architecture}. Number of variables, training speed.
    \item \textit{Time and volume}. 
Bid Feedback - Adx Frequency - hourly
Size - 40M-60M
Events - 15M-32M 
ETL - feature generation
Events - 100M-150M
Frequency - Daily
Size  - 25G-35G
Bidshading Training
8 days look back Adx features
Events = 1B
Frequency - Daily
Size - 280G
Single node training - 8 to 10 hours

    \item \textit{Training pipeline architecture}. Variable selection / variable removal criteria. Presumably the pipeline is eliminating variables that aren't useful; what was the criteria for doing so?
    \item \textit{Training process}. Training process: how expensive is the training process?
    \item \textit{Training pipeline architecture} Details of the training pipeline, data flows, and diagram. 
    \item \textit{Other factors contribute to the final bid price}. Bid shading is only one step of many in a complex DSP system.   
\end{itemize}

Variables that were used in the model, and which ones were often selected. Auction forecasting is an interesting area, and so the question of which variables are selected, and what they do to clearing price, is worth showing I think. It provides some insight into this domain. \\

\begin{itemize}
    \item \textit{Variable contribution}. Variable, R2, Variance contribution. Presumably there should be a lot of variables, eg. url=a.com, etc.
    \item \textit{Model structure}: Show an example win probability model. This would be a table of 
    Variable, Beta parameter (signed), Significance.
    \item \textit{CTR models} There is likely much research on CTR models which use a similar set of variables. Link to this previous literature. Differences to CTR include (A) adding the ln(bidprice) to the winprobability model. (B) This is an AUCTION FORECAST; it is a prediction about what price the auction will clear at. 
    \item \textit{Time of day variables} Time of day variables should be included in the model OR we should create a model for each day-hour of interest. Comments about how time was incorporated. Auctions undergo predictable changes by time.
    \end{itemize}  


\subsection{Model Fit}
\begin{itemize}
    \item \textit{discussion on fit quality}. squared error
    \item \textit{internal numbers}. Internal numbers of fit quality

\end{itemize}    
\subsection{Ad-Server / Real-time evaluation}
\begin{itemize}
    \item \textit{real-time server architecture}. Queries per second. Capping considerations (if worth discussing)
    \item \textit{Data flows and Systems}. 
    \item \textit{Time and Memory consumption}. Time O(log(bidbins)); memory ~ landscape params (How many dummy variables were used?)

\end{itemize}




\subsection{Metrics}
Below we describe a spectrum of metrics used to evaluate performance of the bid shading algorithms from perspectives of regression performance and demand platform performance metrics.

\subsubsection{Regression performance metrics}
Selected metrics for evaluating regression performance of proposed algorithms in this study are:
\begin{itemize}
\item Mean Squared Error (MSE): 
\begin{equation}
 MSE = \frac{1}{N}\sum_{i=1}^{n}(y_i - \hat{y}_i)^2   
\end{equation}
(Smaller is better)
% \item Root MSE (RMSE): $RMSE = \sqrt{MSE}$
\item Coefficient of determination ($r^2$): 
\begin{equation}
 r^2 = \frac{n\Sigma_{xy} - \Sigma_x \Sigma_y}{\sqrt{(n\Sigma_{x^2} - (\Sigma_x)^2)(n\Sigma_{y^2} - (\Sigma_y)^2)}}   
\end{equation}
(Larger is better while $r^2 = 0$ reflects performance of the empirical mean)
\end{itemize}

\subsubsection{Demand platform performance metrics}
The proposed regression task metrics do not encapsulate the most important aspects of the performance of the bid shading system. As discussed in Section~\ref{sec:bid_shading}, the bid shading is actually a process of optimizing the eq.~\ref{eq:surplus_per_response}. To that end we propose the following metrics of evaluation (using the consistent notation) that we will consider the main performance metrics:
\begin{itemize}
    \item Total surplus per bid response: 
    \begin{equation}
        surplus = \sum_{i=1}^{N}(b_i^u - b_i)\mathbf{I}_{B^*}(b_i)
    \end{equation}
    \item Total spend: 
    \begin{equation}
        total\_spend = \sum_{i=1}^{N}b_i\mathbf{I}_{B^*}(b_i)
    \end{equation}
    \item Win rate: 
    \begin{equation}
        win\_rate = \frac{1}{N}\sum_{i=1}^{N}\mathbf{I}_{B^*}(b_i)
    \end{equation}
    \item Cost per mile (CPM): 
    \begin{equation}
        CPM = \frac{1}{N}\sum_{i=1}^{N}b_i\mathbf{I}_{B^*}(b_i)
    \end{equation}
\end{itemize}
All results reported on these metrics shall be percentage improvements or increases as compared to production's non linear bid shading algorithm as absolute numbers could not be disclosed.

\cBl
\subsection{Linear point estimator}

We compare the logistic distribution estimnator to a point estimator.

\begin{equation}
    \mathcal{L} = \frac{1}{N}\sum_{i=1}^{N} \left[(y_i - \Phi_i)^2 * \left|\left\{\begin{matrix} 1 + \alpha & \text{if loss of the bid} \\  1 - \alpha & \text{if win of the bid} \\  \end{matrix}\right. \right| \right].
\end{equation}

The parameter $\alpha \in (0,1)$ indicates the degree of asymmetry. For instance, if $\alpha > 0.5$ the model suffers more loss from under-prediction than from over-prediction. The further $\alpha$ is from 0.5, the more asymmetric the model's preference between under-prediction and over-prediction is.


In this experiment (results shown in Table~\ref{tbl:gamma_impact}) we obtained the highest surplus improvement and the lowest CPM increase at $\gamma = 0.2$ operating point, while the highest total spend and win rate are obtained at $\gamma = 0.8$ operating point, at the cost of the highest CPM increase and lowest surplus improvement. With respect to the criteria described above, we selected $\gamma = 0.2$ as a parameter for all algorithms throughout the experiments.

\subsection{Online experiments and analysis}
Offline experiments are able to show retroactive performance of any bid shading algorithm, however lacking any interaction with the other modules of the system. 
Finally, we discuss performance of the proposed bid shading strategy in the online setting. The two LR and two FM models were deployed on different servers (we removed MLP model due to its poor performance in offline experiments), serving independent traffic and performance was monitored over several days.

% To measure performance of machine learning based bid shading algorithms we deployed LR and FM into a production environment and below we discuss our findings in detail.
% The downside of the offline analysis is that we are not able to measure interactions of bid shader and the system...

\subsubsection{Online A/B test}
In terms of online AB tests, we aggregated results for both LR and FM models and compared them to the randomly selected traffic volume of same scale. Results obtained by the two models as compared to non-linear bid shading approach are given in Figure~\ref{fig:exp_online_ab}. Online results are similar to the offline results in terms of relative ranking of models, with the proposed FM approach being the best one. However, thanks to the online serving control the online setting provided similar or better surplus improvements but at a much lower CPM increase ($< 10\%$ than in the offline counterparts. This behavior is very desirable as the machine learning based bid shading module is capable of playing well into the system providing desired improvements on key metric while not loosing much on other key metrics.
\begin{figure}[!ht]
	\centering
% 	\includegraphics[width=0.44\textwidth]{images/online_results.png}
% 	\caption{Performance metrics improvements and increases (expressed in percentages) for LR and FM model as compared to the nonlinear bid shared collected from separate serving buckets (A/B test).}
 	\label{fig:exp_online_ab}
\end{figure}

\subsubsection{Online A/A/B tests}
To test the stability of the collected results, we separately aggregated performance of the two algorithms across different servers and thus created an A/A/B test. In Figure~\ref{fig:exp_online_aa} we can see that the performance increases compared to the non linear bid shader is very similar between servers running the same algorithm, be it LR or FM model. We can thus further strengthen the claim that the performance measured of any of the algorithms was not a fluke.
\begin{figure}[!ht]
	\centering
% 	\includegraphics[width=0.48\textwidth]{images/online_results_aa_test.png}
% 	\caption{Performance metrics improvements and increases (expressed in percentages) for LR and FM model as compared to the nonlinear bid shading collected from two different servers each showing stability of performance of ML-based approach (A/A/B test).}
	\label{fig:exp_online_aa}
\end{figure}

Finally we ran a similar setup of experiments only per goal type (similarly to the offline counterpart) with sufficient traffic available for the best performing FM model. We can see that across different goal types and across two different servers, the FM model provides very stable and high increase in bid surplus, total spend and win rate, while maintaining relatively low CPM increase ($<10\%$) which is as we discussed earlier a very desirable property.
\begin{figure}[htp]
	\centering
% 	\subfloat{\label{fig:assym_regression1}\includegraphics[width=80mm]{images/online_results_goal_type_a.png}}\hspace{3mm}% % or \hspace{0.3\textwidth}
% 	\subfloat{\label{fig:assym_performance1}\includegraphics[width=80mm]{images/online_results_goal_type_b.png}}
% 	\caption{Performance metrics improvements and increases (expressed in percentages) for the FM model across 6 available goal types as compared to the nonlinear bid shared collected from three separate serving buckets (A/A/B test).}
	\label{fig:exp_online_goal_type_aab}
\end{figure}
With the last online A/A/B test we may conclude that the machine learning based bid shading approach using the FM model is superior to any other approach considered for the demand platform's bidding system, and that it provides a significant value of allowing the strategy equilibrium in the open bid first-price auctions.

\cG

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

